Automated Detection of Antenna Malfunctions in Large-N Interferometers: A Case Study with the Hydrogen Epoch of Reionization Array

We present a framework for identifying and flagging malfunctioning antennas in large radio interferometers. We outline two distinct categories of metrics designed to detect outliers along known failure modes of large arrays: cross-correlation metrics, based on all antenna pairs, and auto-correlation metrics, based solely on individual antennas. We define and motivate the statistical framework for all metrics used, and present tailored visualizations that aid us in clearly identifying new and existing systematics. We implement these techniques using data from 105 antennas in the Hydrogen Epoch of Reionization Array (HERA) as a case study. Finally, we provide a detailed algorithm for implementing these metrics as flagging tools on real data sets.

==> old/corr_metric.tex <==
\section{Correlation Metric\label{ch:corr_metric}}

For each baseline $ij$ the evens and odds are calculated as:
\begin{align}
    \text{even}_{ij} & = (\text{sum}_{ij} + \text{diff}_{ij})/2 \\ 
    \text{odd}_{ij} & = (\text{sum}_{ij} - \text{diff}_{ij})/2
\end{align}
Where $\text{even}_{ij}$ and $\text{odd}_{ij}$ are complex arrays of shape (Ntimes, Nfreqs). Next we normalize the evens and the odds:
\begin{align}
    \text{even\_norm}_{ij} & = \frac{\text{even}_{ij}}{|\text{even}_{ij}|} \\ 
    \text{odd\_norm}_{ij} & = \frac{\text{odd}_{ij}}{|\text{odd}_{ij}|}
\end{align}
And then we calculate the per-baseline correlation metric:
\begin{equation}
    \text{corr\_metric}_{ij} = |\text{mean}(\text{even\_norm}_{ij} \cdot \text{odd\_norm}_{ij}^*)|
\end{equation}
where the user can specify any function to reduce the array along the time and frequency axes, but the default is a mean across the entire array. The per-antenna correlation metric is then simply the mean across all baselines including that antenna:
\begin{equation}
    \text{corr\_metric}_i = \frac{1}{N_j} \sum_{j,j\neq i}{\text{corr\_metric}_{ij}}
\end{equation}
To calculate the cross-polarization metric we take the difference between 4 polarization combinations in the per-baseline correlation metric: $xx-xy$, $xx-yx$, $yy-xy$, $yy-yx$. The mean across all baselines is then taken to get a per-antenna value for all four polarization combinations, and the final per-antenna cross-polarization metric is the maximum value of these four combinations. If the maximum value is less than 0, then the antenna is flagged as being cross-polarized. 

==> old/intro.tex <==
\section{Introduction\label{ch:intro}}

In HERA seasons H1C through the first half of H4C the MeanVij metric was used to diagnose the analog and digital systems. This was then subsequently used as the basis for flagging in downstream analysis and debugging. Now with the introduction of the Phase 2 system, revision to these metrics have been proposed. To minimize the amount of change downstream, this change will be implemented as a revision to the existing metrics; metrics the same name will now be calculated differently. \\
Motivations for this change include:
\begin{itemize}
    \item The Phase 2 RF system has different failure modalities. For example a failed front end and a front-end set to “load” results in a similar power level.
    \item Flagging purely based on statistical deviation assumes a majority of antennas are working. This motivates us to choose a metric where we can specify its desired value.
    \item geographically distributed digitization and Ethernet-based clocks white rabbit clocks increases need for reliable and repeatable correlation metric.
    \item The new correlator bins even and odd samples.
\end{itemize}
Here are some of the questions metrics should answer:
\begin{itemize}
    \item Is an antenna delivering a reasonable gain on the sky?
    \item Is an antenna properly correlating with other antennas?
    \item Is an antenna cross-pol cabled?
\end{itemize}
I would also offer the additional goal of specifying metrics where an desired range can be specified.
